SMILE: Robust Network Localization via Sparse and Low-Rank Matrix Decomposition

Motivated by collaborative localization in robotic sensor networks, we consider the problem of large-scale network localization where location estimates are derived from inter-node radio signals. Well-established methods for network localization commonly assume that all radio links are line-of-sight and subject to Gaussian noise. However, the presence of obstacles which cause non-line-of-sight attenuation present distinct challenges. To enable robust network localization, we present Sparse Matrix Inference and Linear Embedding (SMILE), a novel approach which draws on both the well-known Locally Linear Embedding (LLE) algorithm and recent advances in sparse plus low-rank matrix decomposition. We demonstrate that our approach is robust to noisy signal propagation, severe attenuation due to non-line-of-sight, and missing pairwise measurements. Our experiments include simulated large-scale networks, an 11-node sensor network, and an 18-node network of mobile robots and static anchor radios in a GPS-denied limestone mine. Our findings indicate that SMILE outperforms classical multidimensional scaling (MDS) which ignores the effect of non-line of sight (NLOS), as well as outperforming state-of-the-art robust network localization algorithms that do account for NLOS attenuation including a graph convolutional network-based approach. We demonstrate that this improved accuracy is not at the cost of complexity, as SMILE sees reduced computation time for very large networks which is important for position estimation updates in a dynamic setting, e.g for mobile robots.

==> notes.tex <==
0. more careful use of "Gaussian"
-- we add noise "after converting from RSS" --
we add Gaussian noise to the distance (not the RSS)
noise is Gaussian in dB and log-normal in power and exp(Gaussian) in distance
what is the distribution of (10**(gaussian))**2?
-- square after adding noise --
what does it mean that we square Gaussian noise? mu (chi) = sigma**2 (normal)
intuitively the size of the variance is what doesn't average out 

1. what does this have to do with robotics?
--- low compute times, more suitable for dynamic networks

2. how do we justify uniform NLOS noise?
--- we could model this and see if it's close to uniform
--- black lines in Fig 13 should be gaussian + uniform
--- check if the SMI paper makes assumptions about distribution of S

3. Other noise distributions?
--- what other distributions make sense for this?

4. Compare directly with SDP+exploiting sparsity paper

5. Compare LLE with Isomap?

6. Compare SMI+MLP with SMI+LLE?
--- an MLP trains faster on structured data? stopping training early so that only the low-rank part is learned? --> paper Sampad read (deep image prior)
--- loss on the anchor positions in the middle of the auto encoder and loss on the output "distance matrix"

7. Other ways to learn (replacing both SMI and LLE)
--- train a network on a lot of true distance matrices and see if it can learn to project a noisy distance matrix onto the space of true distance matrices (and see if it learns to encode the true embedding along the way)

8. May be unclear what ||Y||0 is (equation 1)

9. Analyze N more?
If you know sigma, then you're adding a matrix N with some bound on its spectrum. If you know something about the singular values of A and B can you comment on the singular values of A+B? something along the lines of :sigma(A+B) < sigma(A) + sigma(B).
--- gives a bound on how much Gaussian noise we can handle before the noise has too much effect on the rank (or top 2 eigenvectors might change)
sigma1(A * B) =(<=?) sigma1(A) * sigma1(B)
--- with missing measurements, we hadamard product N with something which can only decrease the top singular value so D~ in "missing measurements" might be less altered than D~ above it. Also singular values of binary matrix might concentrate.

10. distance matrix has interesting structure, does bearing matrix?

11. More careful approximation of sparsity estimate
--- we don't adapt the step size of trying to find beta
--- in particular, it might be advantageous to over-estimate beta

-------------------------------------------------------

Results section

Figure 9:
GCN is 200 epochs, but with different size input matrices (matrix multiplication so n cubed but these are sparse)

SMI:
(algorithm1 from the discrete approach paper) In particular, the objective function of (1) is strongly convex for which alternating minimization is known to converge linearly.
% https://link.springer.com/article/10.1007/s11590-021-01753-w
This means
$||f(i+1) - f(*)|| <= c^i ||f(i) - f(*)||$
so I think the time it takes to solve has to do with the initial frobenius norm of O (because X and Y start out as zeros) and the step size (which we scale with n**2).

SMILE:
Least squares complexity
if A is m by n, and we are looking for Ax = b, with m >> n, the complexity is $O(mn^2)$.

LLE complexity
weight matrix construction: $O(DNk^3)$
solve k x k linear equations for N neighborhoods


-------------------------------------------------------
the commonly used non-convex objective function for positive semidefinite matrix completion has no spurious local minima – all local minima must also be global

$f(X) = \frac{1}{2} \sum_{(i,j) \in \Omega}{[M_{i,j} - (X X^T)_{i,j}]^2} $ is not convex, and non-convex algorithms are faster than convex relation algorithms but you have to start with an initialization close to the optimum.

assume no row of Z $(M = ZZ^T)$is too big, then add a regularizer term to $f(X)$ to ensure no row if X is too big.

even if Gaussian noise is added to each entry, when p is large enough (enough entries are present), all local minima are within epsilon of the optimum. 

conclusions are true for noise with std $\sigma$ as long as
$\sigma \leq \frac{mu^2 r}{d \sqrt{\log{d}}}$ where noise can be almost as large as the largest possible entry.

(for many statistical settings that involve missing/noisy data and non-convex regularizers, any stationary point of the non-convex objective is close to global optima)

if the unmasked problem doesn't have spurious local minima then neither does the masked case

--- given this bound on the noise, the output XX.T of something which converges to a locally optimal solution is close to the true ZZ.T (it's close enough by epsilon, so you could rotate to it)
